AMR Dependency Parsing with a Typed Semantic Algebra

We present a semantic parser for Abstract Meaning Representations which learns to parse strings into tree representations of the compositional structure of an AMR graph. This allows us to use standard neural techniques for supertagging and dependency tree parsing, constrained by a linguistically principled type system. We present two approximative decoding algorithms, which achieve state-of-the-art accuracy and outperform strong baselines.

==> parsing-architecture.tex <==
\section{Parsing Architecture}


\subsection{Score prediction}

We use two BiLSTM neural models to predict the scores $\omega$, one for the elementary as-graphs (Figure \ref{fig:nn}a) and one for the operation edges between them (Figure \ref{fig:nn}b). The former is a straightforward neural tagger, the second follows the design of \todo{cite Kiperwasser and Goldberg}\todo{maybe we should stop right here, and just put all the details in section \ref{sec:training}?}. We give a conceptual overview here and present more details and parameters in Section \ref{sec:training}. Both models start out the same: for each word, we generate an input vector $v_i$ that can be e.g. a concatenation of a word embedding and a POS embedding. These vectors get fed into a stack of BiLSTMs, which produce for each position $i$ in the sentence a vector encoding $\textsc{BiRNN}(i)$ of the word in its context. When predicting elementary as-graphs, we simply feed this encoding into a prediction layer to obtain a distribution of scores. For edge-scores $\omega(o[i,j])$, we feed the concatenated encodings $\textsc{BiRNN}(i) \circ \textsc{BiRNN}(j)$ in the prediction layer instead.

